Primary User Emulation and Jamming Attack Detection in Cognitive Radio via Sparse Coding

Cognitive radio is an intelligent and adaptive radio that improves the utilization of the spectrum by its opportunistic sharing. However, it is inherently vulnerable to primary user emulation and jamming attacks that degrade the spectrum utilization. In this paper, an algorithm for the detection of primary user emulation and jamming attacks in cognitive radio is proposed. The proposed algorithm is based on the sparse coding of the compressed received signal over a channel-dependent dictionary. More specifically, the convergence patterns in sparse coding according to such a dictionary are used to distinguish between a spectrum hole, a legitimate primary user, and an emulator or a jammer. The process of decision-making is carried out as a machine learning-based classification operation. Extensive numerical experiments show the effectiveness of the proposed algorithm in detecting the aforementioned attacks with high success rates. This is validated in terms of the confusion matrix quality metric. Besides, the proposed algorithm is shown to be superior to energy detection-based machine learning techniques in terms of receiver operating characteristics curves and the areas under these curves

==> Database <==
\begin{thebibliography}{99}

\bibitem{arjoune2019}
Y.~Arjoune and N.~Kaabouch, ``A comprehensive survey on spectrum sensing in
  cognitive radio networks: Recent advances, new challenges, and future
  research directions,'' \emph{Sensors}, vol.~19, no.~1, p. 126, 2019.

\bibitem{Yucek}
T.~{Yucek} and H.~{Arslan}, ``A survey of spectrum sensing algorithms for
  cognitive radio applications,'' \emph{{IEEE} Commun. Surv. Tuts.}, vol.~11,
  no.~1, pp. 116--130, First 2009.

\bibitem{securcong}
A.~G. {Fragkiadakis}, E.~Z. {Tragos}, and I.~G. {Askoxylakis}, ``A survey on
  security threats and detection techniques in cognitive radio networks,''
  \emph{{IEEE} Commun. Surv. Tuts.}, vol.~15, no.~1, pp. 428--445, First 2013.

\bibitem{jm5738229}
B.~{Wang}, Y.~{Wu}, K.~J.~R. {Liu}, and T.~C. {Clancy}, ``An anti-jamming
  stochastic game for cognitive radio networks,'' \emph{{IEEE} J. Sel. Areas
  Commun.}, vol.~29, no.~4, pp. 877--889, Apr. 2011.

\bibitem{BOUABDELLAH201840}
M.~Bouabdellah, N.~Kaabouch, F.~E. Bouanani, and H.~Ben-Azza, ``Network layer
  attacks and countermeasures in cognitive radio networks: A survey,'' \emph{J.
  Inf. Security Appl.}, vol.~38, pp. 40 -- 49, 2018.

\bibitem{PUEAnSSDF}
D.~Chaitanya and K.~M. Chari, ``Performance analysis of {PUEA} and {SSDF}
  attacks in cognitive radio networks,'' in \emph{Proc. Comp. Commun.,
  Networking Internet Security}.\hskip 1em plus 0.5em minus 0.4em\relax
  Singapore: Springer, 2017, pp. 219--225.

\bibitem{7366825}
F.~{Jin}, V.~{Varadharajan}, and U.~{Tupakula}, ``Improved detection of primary
  user emulation attacks in cognitive radio networks,'' in \emph{Proc. IEEE
  Int. Telecommun. Net. Applications Conf. (ITNAC)}, Nov. 2015, pp. 274--279.

\bibitem{6331677}
Z.~{Yuan}, D.~{Niyato}, H.~{Li}, J.~B. {Song}, and Z.~{Han}, ``Defeating
  primary user emulation attacks using belief propagation in cognitive radio
  networks,'' \emph{{IEEE} J. Sel. Areas Commun.}, vol.~30, no.~10, pp.
  1850--1860, Nov. 2012.

\bibitem{6504232}
L.~{Qian}, X.~{Li}, and S.~{Wei}, ``Cross-layer detection of stealthy jammers
  in multihop cognitive radio networks,'' in \emph{Proc. Int. Conf. Computing,
  Networking Commun. (ICNC)}, Jan 2013, pp. 1026--1030.

\bibitem{rehman2014radio}
S.~U. Rehman, K.~W. Sowerby, and C.~Coghill, ``Radio-frequency fingerprinting
  for mitigating primary user emulation attack in low-end cognitive radios,''
  \emph{IEEE Institution Engr. Technol. (IET) Commun.}, vol.~8, no.~8, pp.
  1274--1284, 2014.

\bibitem{6239877}
W.~{Chin}, C.~{Tseng}, C.~{Tsai}, W.~{Kao}, and C.~{Kao}, ``Channel-based
  detection of primary user emulation attacks in cognitive radios,'' in
  \emph{Proc. IEEE 75th Veh. Technol. Conf. (VTC Spring)}, May. 2012, pp. 1--5.

\bibitem{li2019detecting}
Y.~Li, X.~Ma, M.~Wang, H.~Chen, and L.~Xie, ``Detecting primary user emulation
  attack based on multipath delay in cognitive radio network,'' in \emph{Proc.
  Smart Innovations Commun. and Comput. Sciences}, B.~K. Panigrahi, M.~C.
  Trivedi, K.~K. Mishra, S.~Tiwari, and P.~K. Singh, Eds.\hskip 1em plus 0.5em
  minus 0.4em\relax Singapore: Springer Singapore, 2019, pp. 361--373.

\bibitem{6096448}
N.~T. {Nguyen}, R.~{Zheng}, and Z.~{Han}, ``On identifying primary user
  emulation attacks in cognitive radio systems using non-parametric bayesian
  classification,'' \emph{{IEEE} Trans. Signal Process.}, vol.~60, no.~3, pp.
  1432--1445, Mar. 2012.

\bibitem{4413138}
R.~{Chen}, J.~{Park}, and J.~{H. Reed}, ``Defense against primary user
  emulation attacks in cognitive radio networks,'' \emph{{IEEE} J. Sel. Areas
  Commun.}, vol.~26, no.~1, pp. 25--37, Jan 2008.

\bibitem{123loc}
N.~Patwari and S.~K. Kasera, ``Robust location distinction using temporal link
  signatures,'' in \emph{Proc. 13th Annual ACM Int. Conf. Mobile Comput.
  Networking}, ser. MobiCom '07.\hskip 1em plus 0.5em minus 0.4em\relax New
  York, NY, USA: ACM, 2007, pp. 111--122.

\bibitem{7450851}
W.~R. {Ghanem}, M.~{Shokair}, and M.~I. {Desouky}, ``An improved primary user
  emulation attack detection in cognitive radio networks based on firefly
  optimization algorithm,'' in \emph{Proc. 33rd National Radio Science Conf.
  (NRSC)}, Feb. 2016, pp. 178--187.

\bibitem{liu2009aldo}
S.~Liu, Y.~Chen, W.~Trappe, and L.~J. Greenstein, ``Aldo: An anomaly detection
  framework for dynamic spectrum access networks,'' in \emph{Proc. IEEE Int.
  Conf. Comp. Commun. (INFOCOM)}, 2009, pp. 675--683.

\bibitem{luo2011specific}
Z.~Luo, C.~Lou, S.~Chen, S.~Zheng, and S.~Li, ``Specific primary user sensing
  for wireless security in ieee 802.22 network,'' in \emph{Proc. {IEEE} 11th
  Int. Symp. Commun. \& Inf. Technol. (ISCIT)}, 2011, pp. 18--22.

\bibitem{arul9svm}
S.~Arul~Selvi and M.~Sundararajan, ``{SVM} based two level authentication for
  primary user emulation attack detection,'' \emph{Indian J. Sci. Technol.},
  vol.~9.

\bibitem{8052498}
X.~Zhang, Y.~Ma, Y.~Gao, and S.~Cui, ``Real-time adaptively regularized
  compressive sensing in cognitive radio networks,'' \emph{{IEEE} Trans. Veh.
  Technol.}, vol.~67, no.~2, pp. 1146--1157, Feb. 2018.

\bibitem{choi2017compressed}
J.~W. Choi, B.~Shim, Y.~Ding, B.~Rao, and D.~I. Kim, ``Compressed sensing for
  wireless communications: Useful tips and tricks,'' \emph{{IEEE} Commun. Surv.
  Tuts.}, vol.~19, no.~3, pp. 1527--1550, 2017.

\bibitem{8688400}
M.~{Nazzal}, A.~R. {Ekti}, A.~{Gorcin}, and H.~{Arslan}, ``Exploiting sparsity
  recovery for compressive spectrum sensing: A machine learning approach,''
  \emph{IEEE Access}, vol.~7, pp. 126\,098--126\,110, 2019.

\bibitem{a9020025}
F.~Ye, X.~Zhang, Y.~Li, and H.~Huang, ``Primary user localization algorithm
  based on compressive sensing in cognitive radio networks,''
  \emph{Algorithms}, vol.~9, no.~2, 2016.

\bibitem{7967058}
S.~{Maric}, A.~{Biswas}, and S.~{Reisenfeld}, ``A complete algorithm to
  diagnose and alleviate the effects of physical layer attacks,'' in
  \emph{Proc. Int. Conf. Signals Syst. (ICSigSys)}, May. 2017, pp. 29--34.

\bibitem{7418201}
M.~O. {Mughal}, T.~{Nawaz}, L.~{Marcenaro}, and C.~S. {Regazzoni},
  ``Cyclostationary-based jammer detection algorithm for wide-band radios using
  compressed sensing,'' in \emph{Proc. IEEE Global Conf. Signal Inf. Process.
  (GlobalSIP)}, Dec 2015, pp. 280--284.

\bibitem{davenport2010signal}
M.~A. Davenport, P.~T. Boufounos, M.~B. Wakin, and R.~G. Baraniuk, ``Signal
  processing with compressive measurements,'' \emph{{IEEE} J. Sel. Areas
  Commun.}, vol.~4, no.~2, pp. 445--460, 2010.


\bibitem{8577023p}
E.~C. {Marques}, N.~{Maciel}, and N.~{Naviner}, ``A Review of Sparse Recovery Algorithms,'' in \emph{IEEE Access}, 2019, pp. 1300-1322, vol.7.

\bibitem{ksvd}
M.~Aharon, M.~Elad, and A.~Bruckstein, ``{K-SVD}: An algorithm for designing
  overcomplete dictionaries for sparse representation,'' \emph{IEEE Trans.
  Signal Process.}, vol.~54, no.~11, pp. 4311--4322, Nov. 2006.

\bibitem{machinelearning1}
C.~{Jiang}, H.~{Zhang}, Y.~{Ren}, Z.~{Han}, K.~{Chen}, and L.~{Hanzo},
  ``Machine learning paradigms for next-generation wireless networks,''
  \emph{IEEE Wireless Commun.}, vol.~24, no.~2, pp. 98--105, Apr. 2017.

\bibitem{matlab}
M.~H. Beale, M.~T. Hagan, and H.~B. Demuth, ``{N}eural {N}etwork
  {T}oolbox\texttrademark\hspace{0.1cm}7,'' \emph{User's Guide, MathWorks.}

\bibitem{8509094}
J.~M. {Hamamreh}, H.~M. {Furqan}, and H.~{Arslan}, ``Classifications and
  applications of physical layer security techniques for confidentiality: A
  comprehensive survey,'' \emph{{IEEE} Commun. Surv. Tuts.}, vol.~21, no.~2,
  pp. 1773--1828, Secondquarter 2019.

\bibitem{ompcomp}
B.~L. {Sturm} and M.~G. {Christensen}, ``Comparison of orthogonal matching
  pursuit implementations,'' in \emph{Proc. 20th European Signal Process. Conf.
  (EUSIPCO)}, Aug. 2012, pp. 220--224.


\bibitem{2014arXiv1412.1710H}
K.~{He} and J.~{Sun}, ``{Convolutional Neural Networks at Constrained Time
  Cost},'' \emph{arXiv e-prints}, Dec. 2014.

\bibitem{2}
L.~{Xiao}, L.~J. {Greenstein}, N.~B. {Mandayam}, and W.~{Trappe}, ``Using the
  physical layer for wireless authentication in time-variant channels,''
  \emph{IEEE Trans. Wireless Commun.}, vol.~7, no.~7, pp. 2571--2579, Jul.
  2008.

\bibitem{furqan2018adaptive}
H.~M. Furqan, J.~M. Hamamreh, and H.~Arslan, ``Adaptive {OFDM-IM} for enhancing
  physical layer security and spectral efficiency of future wireless
  networks,'' \emph{Wireless Commun. Mob. Comput.}, vol. 2018, 2018.

\end{thebibliography}

